Zoom: SSD-based Vector Search for Optimizing Accuracy, Latency and Memory

With the advancement of machine learning and deep learning, vector search becomes instrumental to many information retrieval systems, to search and find best matches to user queries based on their semantic similarities.These online services require the search architecture to be both effective with high accuracy and efficient with low latency and memory footprint, which existing work fails to offer. We develop, Zoom, a new vector search solution that collaboratively optimizes accuracy, latency and memory based on a multiview approach. (1) A "preview" step generates a small set of good candidates, leveraging compressed vectors in memory for reduced footprint and fast lookup. (2) A "fullview" step on SSDs reranks those candidates with their full-length vector, striking high accuracy. Our evaluation shows that, Zoom achieves an order of magnitude improvements on efficiency while attaining equal or higher accuracy, comparing with the state-of-the-art.

==> extra.tex <==
\section{Extra}


\paragraph{Comparison of ANN through a table}
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
              & Latency & Accuracy & Memory efficiency \\ \hline
PQ, OPQ, LOPQ & Medium  & Medium   & High              \\ \hline
HNSW          & Low     & High     & Low               \\ \hline
\end{tabular}
\caption{Comparison of different ANN technologies}
\minjia{Add citations and perhaps even more methodologies. Perhaps add another column "SSD" or "Memory-based" and use yes and no to indicate whether they have on-disk index? Also "high dimensionality"?}
\minjia{Change it to 3D coordinates?}
\label{tbl:method-comparison}
\end{table}

% \paragraph{Vector search engine}
% \begin{figure}[H]
% \centering 
% \includegraphics[width=1\linewidth]{figs/semantic-vector-search}
% \caption{The \ANNeX architecture.}
% \minjia{Add ADC reranking}
% \minjia{SSD reranking, changes to "full-length distance computation (FDC) reranking", introduce FDC as how PQ introduces ADC.}
% \minjia{Perhaps it is not necessary required if we can pitch memory efficiency well.}
% \label{fig:overview}
% \end{figure} 

\later{
\paragraph{\textbf{iii) (Optional) Cell-aware data layout shuffling (CLS)}}
\minjia{Does not fit well with the algorithm as well.}

In Section~\ref{}, \ANNeX partitions vector space into multiple cells through a coarse quantizer. After the vector assignment has finished, \ANNeX reorders the layout of the full-length vectors stored in SSDs through the following strategy: a) vectors in the same cell are coalesced together; b) vectors in different cells are scattered away. Vector lengths (\eg, 512-byte) are often smaller than the page size that SSDs load each time. By reordering vectors in the same cell to closer position, it increases the chance of loading multiple vectors into memory with a single SSD read request (\eg, reads a page of 4KB of data).
}

==> impl.tex <==
\paragraph{Implementation}

\paragraph{Implementation.}
Beyond limited distance computation, existing PQ implementation in FAISS has other performance limiting factors, e.g., concurrency synchronization overhead when parallelizing queries with single vector request, which we address in \ANNeX. Since these improvements mostly require good engineering practice than novel methods, we did not discuss them in detail for the interest of space.

We implement the SSD-based post-validation IO using the Linux NVMe Driver. The implementation uses the Linux kernel asynchronous IO (AIO) syscall interface, \code{io\_submit}, to submit IO jobs and \code{io\_getevents} to reap completions of loaded full-length vectors on flash-resident files. Batched requests are submitted through an array of \code{iocb} struct at one. We open the file that stores the full-length vectors in \code{O\_DIRECT} mode to bypass kernel buffers and execute asynchronous IO at sector-level. 
Apart Linux, most modern operating systems, including Windows, allow application to issue asynchronous, batched, and direct IO requests~\cite{linux-aio, windows-aio}.
Apart Linux AIO, there are other userspace NVMe drivers like SPDK~\cite{spdk} and NVMeDirect~\cite{nvme-direct}. We choose AIO for its simplicity and compatibility. 

==> intro-v1.tex <==
\section{Introduction}
\label{sec:intro}

% \minjia{The key is to generate a small set of candidates quickly in-memory and validate only those on SSDs. The introduction should lead to this insight.}
With the blooming of machine learning and deep learning, many information retrieval systems, such as web search, web question and answer, image search, and advertising engine, reply on vector search to find best matches to user queries based on their semantic meaning.  
Take web search as an example.  
%Given a text query message, how can one perform a fast search on a large volume of documents or text passages and accurately retrieve passages that are most relevant to the query based on its \emph{semantic} meaning? 
Traditional document search is mostly based on similarity using bag-of-words and keyword matching, which is difficult to capture the semantic similarity between a query and a document
% the  search engines are mostly based on keywords matching, and it is challenging to understand the searcher's intent from a semantic perspective
~\cite{google-search, bing-search, yahoo-search}? Thanks to the major advances in deep learning (DL) based feature extraction techniques~\cite{dssm, text-similarity-rnn-aaai16}, each text passage now can be represented by a compact fixed-length vector representation.
% , \eg, by leveraging deep learning (DL) based feature extraction techniques~\cite{dssm, text-similarity-rnn-aaai16}. 
Both queries and documents are thus represented as points in high-dimensional vector space whose coordinates are given by their vector values. That makes the semantic similarity search an example of a high-dimensional vector search problem. 
% An enormous amount of computing power may be required to perform this search quickly and accurately.
% To perform this search,

Fig.~\ref{fig:ann-ir-example} compares the traditional way of searching documents versus semantic vector based document retrieval. The vector search engine takes a vector representation of a query and searches a set of data points in a high-dimensional vector space 
% according to a particular distance measure 
(\eg, Euclidean space)~\cite{ann-survey}.  A specified number of document candidates whose vector representations that are close to the query point are retrieved and ranked based on their semantic similarity. 
% through a distance function defined 
Text search is just one example that requires high-dimensional vector similarity search. High-dimensional similarity search also enables solutions to various critical tasks in information retrieval such as online web question-answering and advertising. Furthermore, high-dimensional similarity search is applicable to other data types such as images, tweets, and speech streams.

\begin{figure}[h]
\centering 
\includegraphics[width=1.1\linewidth]{figs/ann-ir-example}
\caption{Example of semantic based vector search.}
\label{fig:ann-ir-example}
\end{figure} 

The simplest search method is linear scan which scans the entire vector database. It computes the distance of each vector in the database to the query, ranks the vectors according to the distance function, and returns the ones with the smallest distance. However, 
% have lead to the construction of information retrieval system based on approximate nearest neighbor (ANN) index. Commercial search engines traditionally employ bag-of-words model for representing a query (or a document) and inverted index for matching~\cite{google-search, bing-search, yahoo-search}. 
% The deep learning based approaches encode compact fixed-length vector representation for input instances (\eg, text passages, or images) using deep neural networks. 
because a vector database can contain millions or even hundreds of millions of vectors, linear scan may not be fast enough to provide interactive queries.
% vector representations enable measuring the degree of semantic equivalence between instances and
That motivates the use of efficient approximate nearest neighbor search (ANN) algorithms for solving the high-dimensional similarity search problem.
% Such advancement is pervasively influencing many applications on text and image retrieval systems, such as search engines, software-as-a-service, social media, image search, online shopping, question-answering systems, recommendation systems, and advertising. 
% For instance, commercial search engines traditionally employ bag-of-words model for representing a query (or a document) and inverted index for matching~\cite{google-search, bing-search, yahoo-search}.
% , which are not effective in capturing semantic understanding. 
% For instance, RNN-based encoder encodes....
% With new semantic vector representation of data, it becomes possible to use efficient approximate nearest neighbor (ANN) search algorithms for the matching phase.
% search deep feature vectors for an encoded query vector. 

% \outline{Semantic similarity search driven? \minjia{Make it an example of ANN usage, but not the entire motivation.}}
% Deep learning (DL) is a fast-growing field pervasively influencing many applications on text, image, and speech processing, including instance retrieval. In contrast to early techniques for instance retrieval based on bag-of-features representations, A DL based approach produces compact fixed-length vector representation for each input instance using deep neural networks, and sends the encoded vector to a serving system to match against millions to billions of candidates. The selected candidates can then be sent to downstream services for further processing (\eg, ranking, answer extraction). 

% Approximate nearest neighbor (ANN) search 
% % Vector search 
% important to many
% % is an emerging technology for 
% % user-facing services 
% tasks such as search engines, software-as-a-service, social media, image search, online shopping, question-answering systems, recommendation systems, and advertising. This algorithm searches a dataset for data points that are close to a query point according to a particular distance measure (\eg, Euclidean distance). 
% to a serving system to match against millions to billions of candidates.
% A vector search engine leverages machine learning models to encode an input (\eg, a text passage, or an image) into a vector, and sends the encoded vector to a serving system to match against millions to billions of candidates using the Approximated Nearest Neighbor (ANN) lookup. 
% A small set of results could then be sent to ranking service for further ranking. 

% has become  today's large-scale, high-performance data-intensive applications. ANN therefore received substantial attention in a variety of domains, both commercial and academic: web-scale search engine, question-and-answering system, recommendation system, image-based search, etc.

% Since the number of instances represented by vectors is humongous and can grow enormously fast, an exhaustive comparison with every candidate is intractable. Thus, finding an instance that is similar or relevant to a given query can be converted to an Approximated Nearest Neighbor (ANN) search in the corresponding feature vector space, which aims at returning the closest vector(s) to the query vector according to a particular distance measure (\eg, Euclidean distance). 

% Therefore, a critical building block for such an instance retrieval system is the Approximated Nearest Neighbor (ANN) search service. 
% Typically ANN search contains two stages: (1) building an ANN index offline for avoiding infeasible exhaustive search, and (2) deploying the constructed ANN index to serve online query requests. 
% Since the number of entities represented by vectors grows enormously fast, the ANN lookup to be scalable and efficient
% % similarity search algorithms 
% to respond queries. 
% \outline{Key challenges or trade-offs?}

% \outline{Low latency and low memory footprint at a fixed accuracy. Apart from this requirement, high accuracy is also important.}
% ANN has been a long-standing research topic, and the low-dimensional case is well-solved~\cite{kd-tree, vp-tree}. Feature vectors extracted by deep learning models often have much higher dimensions and traditional approaches based on the idea of space-partitioning suffers from the "curse of dimensionality", and the complexity of these methods is not more efficient than the brute-force exhaustive distance computation at high dimensional space~\cite{worst-case-kdtree}. As a result, more recent work mainly focus on 
% % obtaining a great trade-off in between low latency and high 
% % accuracy for 
% ANN search in high dimensional space. 

% Existing ANN solutions often target at reducing latency and getting high accuracy. 
% The ANN search is an intrinsically challenging task when used in retrieval systems.
In real-world online services, three aspects of properties of the ANN algorithm are desirable: low latency, high accuracy, and high memory efficiency.
% One big challenge of designing memory-efficient ANN is that its design goal should still aim for low-latency and high accuracy. 
Low latency is crucial because 
% ANN based retrieval system is usually user-facing that comes with stringent service level agreement (SLA). 
online systems often come with stringent service level agreement (SLA) that require responses to be returned within \emph{a few or tens of milliseconds}. Delayed responses could degrade user satisfaction and affect revenue~\cite{reduce-web-latency}. 
High accuracy is expected because the approximation has to return true nearest neighbors with high probability (\eg, >0.90 or >0.95) in order to serve business critical scenarios. 
% Therefore, it is crucial to tap on the overall system performance of ANN index. Unfortunately, state-of-the-art approaches still face major challenges regarding the trade-offs between latency, memory efficiency, and accuracy.
% , ANN service should select most relevant candidates with a high probability (\eg, >0.90 or >0.95 recall). 
% As vector based search becomes more pervasive, the memory efficiency of ANN index can also become very important. 
Memory efficiency is desirable because a memory efficient ANN design is more scalable (\eg, by reducing the number of machines to serve the same amount of request traffic), making an effective use of server resources to amortize the much larger capital expenses (\eg, by allowing co-hosting other services and submitting best-effort batch tasks on the same server~\cite{heracles}) as well as in situations where the available memory is constrained, such as on cloud server and mobile device. 
Therefore, it is crucial to tap on the overall system performance of ANN index. 

Existing ANN approaches still face major challenges regarding the trade-offs between latency, memory efficiency, and accuracy. The state-of-the-art proximity-graph based ANN approaches achieve high accuracy and is fast, but they yield high memory overhead as they need to maintain both the original vectors and additional graph structure in memory~\cite{swg-ann,hnsw}. 
% This memory requirement incurs large Dynamic Random Access Memory (DRAM) footprint and severely limits
% . As ANN scales in both size and importance,  memory efficiency is increasingly becoming one of the important factors for 
% the system scalability and overall cost effectiveness in terms of power and capacity. 
In a separate line of research, quantization-based ANN approaches, in particular product quantization (PQ) and its extensions, support low memory footprint index by compressing vectors into short code, but have worse accuracy~\cite{product-quantization, opq, lopq}. We are thus facing a threefold trade-off between latency, memory efficiency, and accuracy. 
% This paper aims to reconcile all three of these goals.

% , the ANN search should also make an effective use of server resources. 
% In particular, the memory efficiency is often missed by existing ANN designs. 
% Finally, a low DRAM design allows ANN 
% % to meet the latency SLA and accuracy target while allowing 
% best-effort batch tasks to be submitted on the same server to make effective use of server resource~\cite{heracles}. 

% Despite achieving outstanding trade-off between accuracy and latency, few research has taken memory efficiency into account and studied the trade-off between latency, accuracy, and memory. 
% The state-of-the-art proximity-graph based ANN approaches achieve high accuracy and is fast, but they yield high memory overhead as they need to maintain both the original vectors and a full graph structure in memory~\cite{swg-ann,hnsw}. 
% % This memory requirement incurs large Dynamic Random Access Memory (DRAM) footprint and severely limits
% % . As ANN scales in both size and importance,  memory efficiency is increasingly becoming one of the important factors for 
% % the system scalability and overall cost effectiveness in terms of power and capacity. 
% In a separate line of research, quantization-based ANN approaches, in particular product quantization (PQ) and its extensions, support low memory footprint index by compressing vectors into short code, but have mediocre or worse precision~\cite{product-quantization, opq, lopq}.We are thus facing a threefold trade-off between latency, memory efficiency, and accuracy. This paper aims to reconcile all three of these goals.
% which allows to compute the distances between the query and compressed vectors efficiently 
% and allow more vectors in memory at once. However, 
% PQ provides a trade-off between memory usage and accuracy, which makes 
% it possible to 
% However, PQ-based approaches achieve low latency and memory consumption savings at the expense of sacrificing accuracy. 

% \minjia{Problem: The problem I am going to solve is unclear. }

% Furthermore, there are scenarios such as cloud computing servers where the available memory is constrained or the ANN index cannot fit into the memory. 
% Second, ANN search typically scaled across hundreds or thousands of servers. 
% Finally, the memory cost is high and ANN index memory efficiency is increasingly becoming one of the most important factors for overall cost effectiveness. 
% , and an ANN service that cannot provide high accuracy is not quite usable. 
% Key challenges of providing the best ANN service include high accuracy and low latency. 

% We believe that the design of ANN should target the following goals:
% \paragraph{Low latency.} \ANNeX's indexes should respond queries fast enough.
% Rationale: System balance and overall performance.

% \paragraph{High accuracy.}
% Rationale: 

% \paragraph{Memory-efficient indexing.} \ANNeX should use as little memory as possible.m 
% Rationale: DRAM is both more costly and power-hungry per gigabyte than SSD, and its capacity is growing more slowly. 

\minjia{Motivate the importance of DQ as our main result is about DQ improvement.}

% As a point of reference, 
% have different design objectives and often leave aside memory requirement in their design.
% do not include any memory efficiency constraint in their evaluation.
% and they 
% Existing ANN algorithms often target either one or two of aforementioned challenges and 
% , but none achieve all of the goals simultaneously. 
% Table~\ref{tbl:method-comparison} shows the comparison of different ANN technologies. For example,
% As such, 
% as Table~\ref{} shows, is growing more slowly than the capacity of the disk or flash that it indexes. 
% To make ANN indexing more memory efficient, 

% In fact, the higher the compression ratio, the more of reduced recall as there are information loss during compression. As such, existing PQ based approaches often report suboptimal recall than HNSW.

In this paper, we aim to reconcile all three of these goals and propose an architecture, called \ANNeX, that incurs low latency and significantly reduces per-vector memory consumption without sacrificing much accuracy. 
In particular, we build \ANNeX based on a \emph{multi-view} approach: a "preview-step" that happens in-memory, which quickly generates a small set of candidates that have a high probability of containing the true top-K NNs, 
% and requires only a very small number of non-sequential accesses to the disk, and thus performs well on SSDs. 
and a 
% \ANNeX then performs a 
"full-view" step on SSDs to rerank those candidates with their full-length vector information. 
% \ANNeX naturally implements an asynchronous model for the reranking, which has been shown to be more efficient than synchronous computation. We further present our in-memory preview index design, which combines the benefits of both proximity graph based and quantization based approach.

We have evaluated \ANNeX on two different datasets. We also compare the performance of \ANNeX with existing ANN implementations including \IVFPQ and HNSW. Not only we measure traditional metrics such as latency, memory usage, and recall, we also evaluate the DQ metric (Document-Query), which is the product of the document size $D$ (\ie, index memory usage) and query processing rate $Q$ (\ie, the inverse of latency), reflecting overall system efficiency. 
% \minjia{DQ is specifically relates to text data, whereas ANN is more general than dealing with just text.}
% The resulting design fills the gap..., as shown in 

Fig.~\ref{fig:contribution} illustrates the trade-off space among query latency, memory cost, and accuracy (recall). The results of \ANNeX are shown relative to the two baselines. As it shows, \ANNeX offers very good options in the trade-off space among the three factors. \ANNeX achieves much lower latency and higher recall than \IVFPQ with a small sacrifice on memory, improving the DQ metric by 1.7-8.0X and up to 30\% recall improvement. On the other hand, \ANNeX significantly reduces the memory cost while still attaining a similar recall compared to HNSW with slightly higher latency, improving DQ by 3.5--9X with comparable recall. Furthermore, the flexibility provided by \ANNeX allows a user to tailor \ANNeX for different contexts. 
\minjia{One way to support the flexibility claim is to have several configurations of \ANNeX, each focus on different aspect.}
% In particular, 
% The paper looks into the problem of whether there is a possibility to build an ANN system with great trade-offs between latency and accuracy while reducing memory usage. 
% improve memory and latency of PQ based ANN search under a given fixed recall/accuracy.
% presents a new SSD-based ANN system, 
% called \ANNeX, that incurs low latency and significantly reduces per-vector memory consumption without sacrificing much accuracy. 

\begin{figure}[h]
\centering 
\includegraphics[width=1\linewidth]{figs/comparison}
\caption{The \ANNeX contribution.}
\label{fig:contribution}
\end{figure} 



\outline{Challenges.}
% Using this approach, however, poses several challenges. First, how to make the in-memory preview step fast while still being able to generate a sufficiently small candidate set that has a high probability of containing the true NNs. Second, 

\outline{A set of techniques.}

\outline{Results}
\minjia{Summary of two-view approach and SSD validation.}
% Consequently, \ANNeX can saturate the random read I/O on our experimental system, performing 200,000 lookups per second for 512-byte vectors, and it can potentially scale to billions of vectors on a single host. \ANNeX offers several knobs to trade memory efficiency and performance to match available hardware. 


% Solid state drive (SSD) offers large capacity with low cost, yet state-of-the-art ANN search methods are not designed with the full storage hierarchy in mind. 

% Existing ANN systems often rely on DRAM-based indexes. Unfortunately, DRAM is up to 8X more expensive and uses 25X more power per bit than flash, and as Table~\ref{} shows, is growing more slowly than the capacity of the disk or flash that it indexes. As ANN scales in both size and importance, index memory efficiency is increasingly becoming one of the important factors for the system scalability and overall cost effectiveness. In scenarios where memory becomes a concern, \eg, on a cloud computing server where the available memory is constrained or when the database does not fit in RAM, compressed representations of database vectors are used to avoid the bottleneck caused by multiple disk operations when reading data. 



% To the best of our knowledge, no existing ANN systems achieve all of the goals simultaneously. For example, PQ, OPQ, LOPQ. 

% To achieve low latency, high accuracy, and make best use of limited I/O resources, ANN systems require efficient indexes to locate nearest neighbors. 
% To reach these goals, existing ANN systems often rely on DRAM-based indexes. Unfortunately, DRAM is up to 8X more expensive and uses 25X more power per bit than flash, and as Table~\ref{} shows, is growing more slowly than the capacity of the disk or flash that it indexes. As ANN scales in both size and importance, index memory efficiency is increasingly becoming one of the important factors for the system scalability and overall cost effectiveness. In scenarios where memory becomes a concern, \eg, on a cloud computing server where the available memory is constrained or when the database does not fit in RAM, compressed representations of database vectors are used to avoid the bottleneck caused by multiple disk operations when reading data. 

% The compressed representations are typically obtained with product quantization~\cite{product-quantization}, which allows to compute the distances between the query and compressed vectors efficiently. PQ provides a trade-off between memory usage and accuracy, which makes it possible to achieve large memory consumption savings at the expense of reduced recall. In fact, the higher the compression ratio, the more of reduced recall as there are information loss during compression. As such, existing PQ based approaches often report suboptimal recall than proximity graph based approach, such as HNSW~\cite{hnsw}. Furthermore, these solutions still require more than a few bytes per vector in memory with compromised accuracy, and they keep all of the index in memory to avoid disk reads.

% Existing work has examined how to reduce per-vector in-memory index overhead through product quantization and its extensions~\cite{}, but these solutions still require more than a few bytes per vector in memory with compromised accuracy, and they keep all of the index in memory to avoid disk reads.



==> perf-char.tex <==
\section{Performance Analysis}
\label{sec:analysis}

% The IVFPQ design has several system parameters that provide a wide spectrum of trade-off between accuracy, latency, and memory usage
% \minjia{Probably not the right way of describing it because it makes the approach rely on heavy parameter tuning.}

% We characterize the performance of PQ in terms of 1) latency, 2) recall, and 3) \DQ. This study exposes a range of performance issues of the current approach and guides the design of \ANNeX. 
% We produced all of the experimental results presented in this section on a... machine.

% Making these tunable hyperparameters. Perhaps give a table to list out the effect of each?

\minjia{If we move the analysis to after the design, then perhaps some of the insights can be also introduced after the design. The story line becomes "I have a good method that improves 10X, I provide you the design, and now I'm telling you why" instead of "I have some studied some systems and here are some of my observations. Based on these observations, I come up with this design. In other words, my observation justifies my design.  now I'm going to show show that the design actually works." I think the former storyline would work better if I add some high-level intuitive explanation on why certain design choices are made. When it comes to the analysis part, it is just a more formal way to quantify the impact.}

\outline{Performance model + analysis + experiments}

This section presents the performance model of \ANNeX. 
in terms latency, memory overhead, and recall.
It helps exposes a range of performance issues and challenges of the current approach and guides the design of \ANNeX. 
% It then presents several preliminary analysis that have guided the design of the approach introduced later. 
All these evaluations are performed on $X = SIFT1M \in \mathbf{R}^{128}$ on a... machine. 
Table~\ref{tbl:notation} presents the notation used in the analysis. 

\begin{table}[]
\centering
\begin{tabular}{ccc}
Symbol & Meaning                              & Example \\ \hline
       & \underline{IVFPQ parameters}         &         \\
$C_1$     & number of coarse centroids           & $2^{15}$  \\
$C_2$     & number of codewords per sub-dimension & $2^8$    \\
M      & number of sub-dimension              & 32      \\
w	   & number of probes					  & 256     \\
K	   & number of nearest neighbors to retrieve  & 10     \\
       & \underline{Workload characteristics} &         \\
N      & number of database vectors           & 1M      \\
D      & number of dimensions                 & 128     \\
f      & number of bytes of data type         & 4      \\ \hline
\end{tabular}
\caption{Notation.}
\label{tbl:notation}
\end{table}


\outline{HNSW search latency, O(logN), fast, should leverage.}
\outline{Memory overhead, $O(D \times N)$, lead to memory consumption issue.}
\outline{Latency, mostly robust, but occasionally has low recall. Lead to connectivity issue.}

First, we carry out a study on how the number of coarse quantizer centroids affect latency. Our second analysis considers different number of subvectors to encode descriptors and their impact to the recall, latency, and memory footprint. Finally, we carry out an evaluation on the size of candidate sets that contain top-K NNs. This leads us to identify appealing choices for our ANN design. 

% \outline{Existing PQ codebook based search, lookup-sum.}
% Existing PQ based ANN systems such as FAISS implements PQ as IVFPQ: as shown in Listing~\ref{} to avoid exhaustive search. 

% In PQ, we denote:
% \begin{itemize}
% \item N: the number of database vectors;
% \item D: the number of dimensions;
% \item C1: the number of coarse centroids;
% \item C2: the number of quantization per sub-vector;
% \item M: the number of sub-vectors;
% \item f: the number of bytes of data type, \eg, f = 4 when the data type is float.
% \end{itemize}

% The size of the database is $N \times D \times f$. The size of coarse centroid codebook is $C1 \times D \times f$. The size of the product quantization codebook is $C2 \times D \times f$. 

\paragraph{Per-query latency}
A query first searches the IVFPQ coarse quantizer centroids to find closest cells that are the closest to the query, and the search scans  vectors in selected cells to find top-K NNs. The execution time of serving a query vector can be estimated as 

\begin{equation} \label{eq1}
\begin{split}
Time & = Finding\ closest\ cells\ time\ (FC) \\
 & + Populating\ PQ\ lookup\ table\ time\ (PL) \\
 & + Scanning\ selected\ cells\ time\ (SC) 
\end{split}
\end{equation}
\minjia{Instead of listing out the analysis as PQ's analysis, I might as well change the FC step so the entire section becomes an analysis of \ANNeX. }

% \begin{eqnarray*}
% \!\begin{aligned}
% Time = Find\ centroid\ time \\ \nonumber
% +\ Sub\-distance\ calculation\ for\ populating\ PQ\ lookup\ table \\ \nonumber
% + Actual\ distance\ calculation\ using\ sub-distance \\ \nonumber
% calculation\ result\ (codebook\ Lookup +\ sum\ up\ subdistances).  \\ \nonumber
% \end{aligned}
% \end{eqnarray*}

The execution time of finding closest cells is an linear scan of coarse quantizer centroids to find $w$ cells to probe into. Its execution time can be estimated as a function of the data reuse using the roofline model as
\begin{equation} \label{eq2}
\begin{split}
FC & = Max(Compute, DataTransfer) \\
 & = Max(\frac{2 \times C_1 \times D}{ComputePeak}, \frac{C_1 \times D \times f}{Bandwidth(C_1 \times D \times f)}) \\
\end{split}
\end{equation}

% \begin{eqnarray}
% Find\ centroid\ time = Max(Compute, DataTransfer) \\ \nonumber
% = Max(\frac{2 \times C1 \times D}{ComputePeak}, \frac{C1 \times D \times f}{Bandwidth(C1 \times D \times f)})
% \end{eqnarray}

Before probing into each selected cell, IVFPQ precomputes sub-distance for populating PQ lookup table that is used for quickly measuring the distance between a query and quantized vectors. The execution time of this precomputation step is
\begin{equation} \label{eq3}
\begin{split}
PL & = Max(Compute, DataTransfer) \\
 & = Max(\frac{2 \times C_2 \times D}{ComputePeak}, \frac{C_2 \times D \times f} {Bandwidth(C_2 \times D \times f)})  \\
\end{split}
\end{equation}

% \begin{eqnarray}
% Subdistance\ calculation\ for\ PQ\ Table \\ \nonumber
% = Max(Compute, Data Transfer) \\ \nonumber
% = Max(\frac{2 \times C2 \times D}{ComputePeak}, \frac{C2 \times D \times f} {Bandwidth(C2 \times D \times f)}) 
% \end{eqnarray}

% centroids and sub-distance calculation for PQ table 

Once the precomputation has been done, the next step is to scan compressed vectors in selected cells through ADC (asymmetric distance calculation), which calculates actual distance by looking up the codebook and summing up sub-distances. Assume summing up sub-distance is fast as it sits in L2 or even L1 cache, the execution time. 
\begin{equation} \label{eq4}
\begin{split}
SC & = Max(Compute, DataTransfer) +\ maintain\ heap \\
 & = w \times Max(\frac{\frac{N}{C_1} \times M}{ComputePeak}, \frac{\frac{N}{C_1} \times M \times log(C_2)}{8 \times Bandwidth (\frac{N}{C_1} \times M \times \frac{log(C_2)}{8})} \\
 & + (N \times \frac{w}{C1} \times log(K)) \\
\end{split}
\end{equation}
% \begin{eqnarray}
% Actual\ Distance\ Calculation\ Time \\ \nonumber
% = Max(Compute, DataTransfer) + maintain heap \\ \nonumber
% = w \times Max(\frac{\frac{N}{C_1} \times M}{ComputePeak}, \frac{\frac{N}{C_1} \times M \times log(C_2)}{8 \times Bandwidth ( N \times M \times \frac{log(C_2)}{8})} + (N \times \frac{w}{C1} \times log(K))
% \end{eqnarray}

\minjia{Explain ComputePeak and Bandwidth. The goal is to come up an example that shows it is impossible to get a few millisecond latency if C1 is not large.}

% For adding subsum
% \begin{eqnarray}
% (n/c1 * m * 4 bytes)/Bandwidth()
% \end{eqnarray}

The execution time is decided by both the compute time and the data transfer time. 
\paragraph{Memory overhead.} For IVFPQ, the total memory overhead (MO) required to store the data is given by 
\begin{equation} \label{eq5}
\begin{split}
MO & = Compressed\ vectors \\
   & + Coarse\ quantizer\ centroids + PQ\ codebook \\
   & = N \times M \times \frac{log(C_2)}{8} \\
   & + C_1 \times D \times f + C_2 \times D \times f
\end{split}
\end{equation}

As modern computers often bottleneck on memory bandwidth, \eg, the bandwidth of the experimental machine has a memory bandwidth of 59GB/s, which is less than XX\% of the machine's peak compute performance 1.69Tflops, and because of the lookup-add operation for calculating the ADC, the IVFPQ approach, in particular the SC step, is memory bandwidth bounded instead of compute bounded. 

% Explanation and analysis
When $C_1$ is relatively small, the computation time and data transfer time of FC is also small (Equation~\ref{eq2}), whereas the SC execution time is large as for a given number of probes $w$, smaller $C_1$ indicates that there are more vectors to scan (Equation~\ref{eq4}).
When $C_1$ is large, as the FC execution time is linear in $C_1$ and there are less vectors to scan at SC (for a fixed $w$), the complexity of the entire execution time starts to be dominated by FC. 
\textbf{Challenge:} Exact search of coarse quantizer centroids can become a bottleneck as $C_1$ increases.
% Modern architecture has limited memory bandwidth. Given the bandwidth of 59GB/s, it is difficult to reach a few milliseconds latency given these amount of memory accesses.

\paragraph{Tradeoffs: Accuracy/Latency/Memory.}

The higher the number of $C_1$ centroids, the fewer then number of data points we need to scan to achieve a desired level of accuracy. In extreme, when the number of centroid is equal to the number of data points, then   we simply need to scan K-data points to find K-NN. 
% However, notice that we also need to scan all the centroids.
For the same number of $C_2$ centroids, the lower the M, the better accuracy and larger memory saving, but also the worse accuracy. This is because...
$C_2$ is generally very small (\eg, 256) so the $C_2$ codebook size is trivial.
Key observation: The approximated top-most NN might not always match the exact top-most NN, but the top-most NN is more likely to fall within the top-R (e.g., R = 10) results.

\paragraph{Example.}

Assume....
The default memory requirement is $1 million \times 128 \times 4$.
By Equation~\ref{eq5}, the memory requirement is 
$1 million \times (M \times \frac{Log(C_2)}{8})  + C_1 \times 128 \times 4 + C_2 \times 128 \times 4$. Assume the memory constraint is 1GB, we can use our performance model to get a configuration. We want to maximize recall while staying within 1ms and staying under 1GB of memory requirement. 
From this analysis, we can come up with the observation that we can use large C1 (\eg, C1 = 65536) as its size is still much smaller than the compressed representation of vectors. 

We use our memory and performance model for PQ along with our understanding of accuracy trend to answer this question. 
Choosing C1 : Our performance model shows that when C1 = 14000, the centroid time is 0.114ms. This is already larger than our total latency budget so C1 larger than 14000 can be safely ignored. When C1 = 10,000, our centroid latency is 0.08ms. So we can start our search around with this value.  
Choosing m and C2 : Now the largest value of m is 100 and largest supported value of C2 = 256. Using these two values,  and C1 = 10,000. The memory requirement is 1.49 GB which is well under our memory requirement. 
Now we can find a w (number of probes) that gives us the required accuracy. If the centroid scan time is the performance bottleneck, then we can now reduce the centroid to reduce the latency.


% \paragraph{Accuracy:}
% The key insight are three folds 

% 	1) The higher the number of C1 centroids, fewer then number of data points we need to scan to achieve a desired level of accuracy. In extreme, when the number of centroid is equal to the number of data points, then   we simply need to scan k-data points to find k-NN. However, notice that we also need to scan all the centroids.
% 	2) For a given number of probes, the accuracy increases as we decrease the number of centroids.
% 3) For the same number  of C2 centroids, higher the m, better the PQ accuracy.  
% Indication:

% \outline{Top-K falls into top-R}

% \paragraph{Observation 3.} For the same number  of C2 centroids, higher the m, better the PQ accuracy.  



% \subsection{Small K vs. Large K of coarse quantizer}
% \outline{Large codebook improves recall but causes first level overhead.}
% \paragraph{Observation 1} The higher the number of C1 centroids, fewer then number of data points we need to scan to achieve a desired level of accuracy. In extreme, when the number of centroid is equal to the number of data points, then   we simply need to scan k-data points to find k-NN. However, notice that we also need to scan all the centroids.
% For a given number of probes, the accuracy increases as we decrease the number of centroids.

% \minjia{Add the on-the-paper analytics here as well.}




==> put-it-all-together.tex <==
\section{\ANNeX Configuration}
\label{sec:analysis}

% \minjia{If we move the analysis to after the design, then perhaps some of the insights can be also introduced after the design. The story line becomes "I have a good method that improves 10X, I provide you the design, and now I'm telling you why" instead of "I have some studied some systems and here are some of my observations. Based on these observations, I come up with this design. In other words, my observation justifies my design.  now I'm going to show show that the design actually works." I think the former storyline would work better if I add some high-level intuitive explanation on why certain design choices are made. When it comes to the analysis part, it is just a more formal way to quantify the impact.\minjia{Made changes accordingly.}}

% \subsection{Balancing Latency, Memory-Efficiency, and Accuracy}
% \label{subsec: balancing}
The latency, recall, and memory cost of \ANNeX depend on a set of parameters:
% \ANNeX's goals of low query latency, low memory usage, and high accuracy are impacted by the parameters in \ANNeX: 
\Ncluster, the number of \cells; $M$, the number of sub-dimension of product quantization we use to encode vectors; $efSearch$, the size of the search queue at the routing layer; $Nscan$, the number of selected \cells to scan; and $R$, the size of the candidate list.
The effect of these five parameters is intertwined. Table~\ref{tbl:hyperparameters} shows their impact to query latency, recall, and memory cost.
% Table~\ref{tbl:hyperparameters}.
% $C_{coarse}$ and $M$ both are build-time parameters that must be set when the index is built. They impact query latency, memory efficiency, and accuracy. $Nscan$, $efSearch$, and $R$ are search time parameters that can be adjusted before performing ANN search. They impact query latency and accuracy. 
\begin{table}[H]
\begin{tabular}{|r|c|c|c|}
\hline
              			& Latency & Recall & Memory cost \\ \hline
\Ncluster $\uparrow$ 	& $T_{CS} \uparrow T_{VS} \downarrow$   & $\uparrow$    & $\uparrow$             \\ \hline
M $\downarrow$              & $T_{VS} \downarrow$     & $\downarrow$     & $\downarrow$ $\downarrow$            \\ \hline
efSearch $\uparrow$       & $T_{CS}\uparrow$   & $\uparrow$    & ---              \\ \hline
Nscan $\uparrow$          & $T_{VS}\uparrow$   & $\uparrow$    & ---              \\ \hline
R $\uparrow$              & $\uparrow$   & $\uparrow$    & ---              \\ \hline
\end{tabular}
\caption{Impact of \ANNeX system parameters to latency, recall, and memory cost. Double arrows indicate a significant impact.}
\label{tbl:hyperparameters}
\end{table}


% \paragraph{Parameter selection:} 
% 
To navigate the combinatorial space of these parameters that offer effectiveness and efficiency while still meeting specific latency, memory, and accuracy targets, 
% To navigate the combinatorial space of options for these parameters, 
we adopt an iterative two-step approach. 
\minjia{Need to revise based on the "effectiveness" and "efficiency".}

In the first step, \ANNeX chooses \Ncluster and $M$ for a memory cost target (MOT). The memory cost of \ANNeX is calculated as:
% which is given by: 
% \begin{thm}
% The total memory overhead (MO) required to store the \ANNeX index is given by 
\begin{equation} \label{eq5}
\begin{split}
% MOT & = size\ of\ quantized\ vectors \\
%    & + size\ for\ caching\ distance\ terms \\
%    & + size\ of\ PQ\ codebook \\
% %    & + size\ of\ cluster\ centroids \\
%    & + size\ of\ routing\ layer  \\
MOT & = N \times( M \times \frac{log(L)}{8\textnormal{-}bit} + 4)  + L \times D \times f \\
%    & + N_{cluster} \times (D + \frac{OutD}{OutD-1}) \times f
   & + N_{cluster} \times (D + OutD) \times f
%    + L \times D \times f + N_{cluster} \times \frac{OutD}{OutD-1} \times f
\end{split}
\end{equation}
where each entry in \ANNeX uses $M \times \frac{log(L)}{8\textnormal{-}bit} + 4$ bytes (log(L) bits for the PQ code of each sub-dimension, and 4 bytes for caching the precomputation result). The codebook uses $L \times D \times f$ bytes. The routing layer requires $N_{cluster} \times (D + OutD) \times f$ bytes to store.
% \end{thm}
% \begin{proof}
% % $C_2$ is generally very small (\eg, 256) so the $C_2$ codebook size is trivial.
% Before scanning each selected cell, \ANNeX has already precomputed all possible sums of terms (\eg, the second and the fourth term in Equation 8~\ref{}) 
% and stored those results in an LUT 
% % and populating PQ lookup table that is used 
% for quickly measuring the distance between a query and quantized vectors. 
% \end{proof}

In the next step, \ANNeX iterates through the values of $efSearch$, $N_{scan}$, and $R$ to select the combination of values that meet the recall target while maximizing a cost function that expresses the system efficiency as \emph{VQ} (Vector--Query), inspired by the DQ (Document--Query) metric from web search engine~\cite{bitfunnel}.
% In this paper, we also employ
% VQpropose a new evaluation metric---the 
% \emph{VQ} (Vector--Query) metric as an important cost metric for ANN, inspired by the DQ (Document--Query) metric from web search engine~\cite{bitfunnel}. 
VQ is defined
% which measures the overall efficiency of an ANN algorithm 
as the product of the number of vectors per machine and the queries per second. 
It measures the
% Recall that the goal of \ANNeX is to improve
the overall ANN system efficiency and has a direct impact on the number of machines and cost to serve ANN. The lower the latency and memory cost, the higher the VQ. On the other hand,
% based on balancing the query latency and recall and selecting only those values that meet the query latency and recall target. 
if no combinations can meet the recall target, \ANNeX increases the MOT and repeats from the first step. 
% For example, picking a larger $M$ will increase the memory cost, but it will make the preview index more accurate and increases the likel
% The size of the candidate list $R$ obviously needs to be at least equal or lager than $K$. A typical way to select it is to aim at balancing the cost of random read accesses on SSD with the recall.
In this iterative process, \ANNeX collaboratively optimizes query latency, memory cost, and recall by selecting the configuration that maximizes the VQ metric for a given recall target.
% These parameters provide the flexibility for \ANNeX to fit different targets based on the application's preferences. 
% \minjia{Pitch the work in the optimization space instead of the trade-off space.}


% \ANNeX also allows other configurations based on the the application's preferences and query rate. The hyperparameters provide the flexibility for \ANNeX to fit different targets. 
% , and it chooses  and iterates $Nscan$ to select values that meet the recall target. In the next step, \ANNeX reduces $M$ and chooses $efSearch$ and $R$ that still meet the recall and latency requirement. Alternatively, the parameter can be optimized using black-box hyperparameter tuners such as Google Vizier~\cite{google-vizier} or Hyperdrive~\cite{hyperdrive}.
% , which support exploration and exploitation of the search space with grid search, bandit search, Gaussian optimization based search, etc.

% \paragraph{Trading off :}
% We want to choose large $C_{coarse}$ so that \ANNeX scans fewer preview vectors to reach the same accuracy. The smaller the $M$, the more compression we get on the preview index size. However, if $M$ is too small, we lose too much precision, and that can increase the size of candidates $R$ at the full-view step. Larger $Nscan$ leads to higher latency, but it also increases the accuracy.



% \begin{table}[]
% \begin{tabular}{|l|l|l|l|}
% \hline
%               & Latency & Accuracy & Memory efficiency \\ \hline
% $C_{coarse}$  & \cmark   & \cmark    & \cmark             \\ \hline
% M             & \cmark   & \cmark    & \cmark             \\ \hline
% efSearch      & \cmark   & \cmark    & \xmark              \\ \hline
% Nscan         & \cmark   & \cmark    & \xmark              \\ \hline
% R             & \cmark   & \cmark    & \xmark              \\ \hline
% \end{tabular}
% \caption{Impact of hyperparameters}
% \label{tbl:hyperparameters}
% \end{table}



\outline{Performance model + analysis + experiments}

% \subsection{Performance Analytics}
% \label{subsec: analytics}

% This section presents the performance analytics of \ANNeX. \minjia{What does this model do and provide?} 



% \outline{HNSW search latency, O(logN), fast, should leverage.}
% \outline{Memory overhead, $O(D \times N)$, lead to memory consumption issue.}
% \outline{Latency, mostly robust, but occasionally has low recall. Lead to connectivity issue.}

% \minjia{Some of these analysis are put into the challenge section. The most important one is the large codebook of coarse quantizer and top-K falls into top-R. Those are already included to justify our design. So here this paragraph can be removed.}
% First, we carry out a study on how the number of coarse quantizer centroids affect latency. Our second analysis considers different number of subvectors to encode descriptors and their impact to the recall, latency, and memory footprint. Finally, we carry out an evaluation on the size of candidate sets that contain top-K NNs. This leads us to identify appealing choices for our ANN design. 

% \outline{Existing PQ codebook based search, lookup-sum.}
% Existing PQ based ANN systems such as FAISS implements PQ as IVFPQ: as shown in Listing~\ref{} to avoid exhaustive search. 

% In PQ, we denote:
% \begin{itemize}
% \item N: the number of database vectors;
% \item D: the number of dimensions;
% \item C1: the number of coarse centroids;
% \item C2: the number of quantization per sub-vector;
% \item M: the number of sub-vectors;
% \item f: the number of bytes of data type, \eg, f = 4 when the data type is float.
% \end{itemize}

% The size of the database is $N \times D \times f$. The size of coarse centroid codebook is $C1 \times D \times f$. The size of the product quantization codebook is $C2 \times D \times f$. 

% \begin{algorithm}[h!]
% \caption{\hfill \ANNeX in-memory index construction algorithm}
% \label{algo:index-build-step}
%   \begin{algorithmic}[1]
%     \State \textbf{Input:} Training set $Y$, vector dimension $D$.
%     	\label{lst:preview-step:input}
%     \State \textbf{Output:} An \ANNeX index \emph{index}.
%     	\label{lst:preview-step:output}
%     \State \textbf{Hyperparameter:} Number of subspaces $M$, number of sub-codewords $k$ in each sub-codebook, size of codebook of coarse quantizer $C_1$.
%     	\label{lst:preview-step:hyperparameter}        
%     \State $index.compressed\_layer.C_1 \leftarrow clustering(Y, D, |C_1|)$
% 		\Comment{ Generate the codebook of coarse quantizer using Lloyd's algorithm.}
%         \label{lst:preview-step:routing} 
%     \ForAll {$i$ \textbf{in} 0..($|Y|-1$)}
%     	\State $id, codeword \leftarrow assign(Y[i], index.C_1)$ 
%     	\State $R[i] \leftarrow compute\_residual(Y[i], codeword)$ 
%         \label{lst:preview-step:generate-candidate-set} 
%     \EndFor    
%     \ForAll {$i$ \textbf{in} 0..($M-1$)}
%     	\State $index.compressed\_layer.C_2[i] \leftarrow train\_residual(R[:i \times D/M, (i + 1) \times D/M], k)$ 
%         \label{lst:preview-step:generate-candidate-set} 
%     \EndFor   
%     \ForAll {$i$ \textbf{in} 0..($|Y|-1$)}
%     	\State $id, codeword \leftarrow assign(Y[i], index.C_1)$ 
%         \State $Y_{pq\_code}[i] \leftarrow product\_quantizer(R[i])$
%     	\State $index.compressed\_layer.lists[i].add(Y_{pq\_code}[i])$
%         \label{lst:preview-step:generate-candidate-set} 
%     \EndFor  
%     \ForAll {$i$ \textbf{in} 0..($|Y|-1$)}
%     	\ForAll {$m$ \textbf{in} 0..($|M|-1$)}
%         	\State $precompute\_table[i] \leftarrow 2 \times \|r_m\|^2 + 2 \times \langle c_m, r_m \rangle$ 
%         	\label{lst:preview-step:generate-candidate-set} 
%         \EndFor
%     \EndFor
%     \State $index.routing\_layer \leftarrow CreateHnsw(C_1, M)$
%     \State $index.routing\_layer.connectivity\_augmentation()$
%   \end{algorithmic}
% \end{algorithm}

% \minjia{The first term is for computing the first term of ADC. This perhaps can help explain why we see increased execution time as w increases.}
% \paragraph{Memory overhead.} For IVFPQ, the total memory overhead (MO) required to store the data is given by 
% \begin{equation} \label{eq5}
% \begin{split}
% MO & = Compressed\ vectors \\
%    & + Coarse\ quantizer\ centroids + PQ\ codebook \\
%    & = N \times M \times \frac{log(C_2)}{8} \\
%    & + C_1 \times D \times f + C_2 \times D \times f
% \end{split}
% \end{equation}
% $C_2$ is generally very small (\eg, 256) so the $C_2$ codebook size is trivial.



% \minjia{Many of these analysis perhaps can be described as Lemmas or even Theorems in the design. We should give some Lemma on the memory usage of \ANNeX.}

% \begin{algorithm}[h!]
% \caption{\hfill \ANNeX online search algorithm}
% \label{algo:preview-step}
%   \begin{algorithmic}[1]
%     \State \textbf{Input:} Query vector $q$, \ANNeX in-memory index $\emph{index}$, number of nearest neighbors $K$ to retrieve.
%     	\label{lst:preview-step:input}
%     \State \textbf{Output:} Top-$K$ nearest neighbors.
%     	\label{lst:preview-step:output}
%     \State \textbf{Hyperparameter:}  The number of cells to scan $nScan$, size of candidate short-list $W$.
%     	\label{lst:preview-step:hyperparameter}
%     \State \textbf{Initialization:}  
%     	\State $W \leftarrow min\_priority\_queue(|W|)$ 
%     	\label{lst:preview-step:hyperparameter}
%     \State $I^{nScan}, D^{nScan} \leftarrow index.routing\_layer.search(q, nScan)$
% 		\Comment{ Return top-$nScan$ cells with minimal distance to $q$.}
%         \label{lst:preview-step:routing} 
%     \ForAll {$i$ \textbf{in} 0..($nScan-1$)}
%     	\State $selected\_cell \leftarrow index.compressed\_layer.list[n]$
%     	\ForAll {$n$ \textbf{in} 0..($selected\_cell.size-1$)}
%           \State $dist \leftarrow compute\_ADC(selected\_cell[n])$ 
%           \State $W.add(dist, selected\_cell[n].id)$ 
%           	\label{lst:preview-step:generate-candidate-set}
%         \EndFor
%     \EndFor    
%   \end{algorithmic}
% \end{algorithm}

% A query first goes through the routing layer to search cells that are the closest to the query. For those selected cells, \ANNeX scans compressed vectors in those cells to obtain a candidate set of top-R NNs. The top-R NNs are reranked with full-length vectors stored in SSDs to get the final top-K NNs. 
% he execution time of serving a query vector is therefore estimated as 

% \begin{equation} \label{eq1}
% \begin{split}
% Time & = Cluster\ finding\ time\ (CF) \\
% %  & + Populating\ lookup\ table\ time\ (PL) \\
%  & + Vector\ scanning\ time\ (VS) \\
%  & + SSD\ reranking\ time\ (RE) 
% \end{split}
% \end{equation}
% \minjia{Instead of listing out the analysis as PQ's analysis, I might as well change the FC step so the entire section becomes an analysis of \ANNeX. }

% \begin{eqnarray*}
% \!\begin{aligned}
% Time = Find\ centroid\ time \\ \nonumber
% +\ Sub\-distance\ calculation\ for\ populating\ PQ\ lookup\ table \\ \nonumber
% + Actual\ distance\ calculation\ using\ sub-distance \\ \nonumber
% calculation\ result\ (codebook\ Lookup +\ sum\ up\ subdistances).  \\ \nonumber
% \end{aligned}
% \end{eqnarray*}

% The execution time of finding closest cells takes logarithmic time to search $C_1$ centroids of the coarse quantizer and to find $w$ cells to probe into. Its execution time is $O(log(C_1))$.
% can be estimated as a function of the data reuse using the roofline model as
% \begin{equation} \label{eq2}
% \begin{split}
% FC & = Max(Compute, DataTransfer) \\
%  & = Max(\frac{2 \times C_1 \times D}{ComputePeak}, \frac{C_1 \times D \times f}{Bandwidth(C_1 \times D \times f)}) \\
% \end{split}
% \end{equation}

% \begin{eqnarray}
% Find\ centroid\ time = Max(Compute, DataTransfer) \\ \nonumber
% = Max(\frac{2 \times C1 \times D}{ComputePeak}, \frac{C1 \times D \times f}{Bandwidth(C1 \times D \times f)})
% \end{eqnarray}

\later{
\begin{thm}
The resulting \ANNeX index retrieves top-$K$ approximate nearest neighbors in expected time: 
\begin{equation} \label{eq1}
\begin{split}
Time & = Cluster\ finding\ time\ (CF) \\
%  & + Populating\ lookup\ table\ time\ (PL) \\
 & +\ Vector\ scanning\ time\ (VS) \\
 & +\ SSD\ reranking\ time\ (RE) 
\end{split}
\end{equation}
where 
\begin{equation} \label{eq4}
\begin{split}
SC & = Max(Compute, DataTransfer) +\ maintain\ heap \\
 & = w \times D +  \times Max(\frac{\frac{N}{C_1} \times M}{ComputePeak}, \frac{\frac{N}{C_1} \times M \times log(C_2)}{8 \times Bandwidth (\frac{N}{C_1} \times M \times \frac{log(C_2)}{8})}) \\
 & + N \times \frac{w}{C1} \times log(K) \\
\end{split}
\end{equation}
\end{thm}
\begin{proof}
The execution time of finding closest cells takes logarithmic time to search $C_1$ centroids of the coarse quantizer and to find $w$ cells to probe into. Its execution time is $O(log(C_1))$.
When scanning compressed vectors, distance is measured by 
% Once the precomputation has been done, the next step is to scan compressed vectors in selected cells through ADC (asymmetric distance calculation), which calculates actual distance by 
looking up the LUTs and summing up precomputed sub-distances. 
\end{proof}
}

% The execution time of this precomputation step is
% \begin{equation} \label{eq3}
% \begin{split}
% PL & = Max(Compute, DataTransfer) \\
%  & = Max(\frac{2 \times C_2 \times D}{ComputePeak}, \frac{C_2 \times D \times f} {Bandwidth(C_2 \times D \times f)})  \\
% \end{split}
% \end{equation}

% \begin{eqnarray}
% Subdistance\ calculation\ for\ PQ\ Table \\ \nonumber
% = Max(Compute, Data Transfer) \\ \nonumber
% = Max(\frac{2 \times C2 \times D}{ComputePeak}, \frac{C2 \times D \times f} {Bandwidth(C2 \times D \times f)}) 
% \end{eqnarray}

% centroids and sub-distance calculation for PQ table 

% Assume summing up sub-distance is fast as it sits in L2 or even L1 cache, 
% The execution time can be estimated as a function of the data reuse using the roofline model as
% \begin{equation} \label{eq4}
% \begin{split}
% SC & = Max(Compute, DataTransfer) +\ maintain\ heap \\
%  & = w \times D +  \times Max(\frac{\frac{N}{C_1} \times M}{ComputePeak}, \frac{\frac{N}{C_1} \times M \times log(C_2)}{8 \times Bandwidth (\frac{N}{C_1} \times M \times \frac{log(C_2)}{8})}) \\
%  & + N \times \frac{w}{C1} \times log(K) \\
% \end{split}
% \end{equation}
% \begin{eqnarray}
% Actual\ Distance\ Calculation\ Time \\ \nonumber
% = Max(Compute, DataTransfer) + maintain heap \\ \nonumber
% = w \times Max(\frac{\frac{N}{C_1} \times M}{ComputePeak}, \frac{\frac{N}{C_1} \times M \times log(C_2)}{8 \times Bandwidth ( N \times M \times \frac{log(C_2)}{8})} + (N \times \frac{w}{C1} \times log(K))
% \end{eqnarray}

% \minjia{Explain ComputePeak and Bandwidth. The goal is to come up an example that shows it is impossible to get a few millisecond latency if C1 is not large. \minjia{No longer applies.}}

% For adding subsum
% \begin{eqnarray}
% (n/c1 * m * 4 bytes)/Bandwidth()
% \end{eqnarray}

% The execution time is decided by both the compute time and the data transfer time. As modern computers often bottleneck on memory bandwidth, \eg, the bandwidth of the experimental machine has a memory bandwidth of 59GB/s, which is less than XX\% of the machine's peak compute performance 1.69Tflops, and because of the lookup-add operation for calculating the ADC, the IVFPQ approach, in particular the SC step, is memory bandwidth bounded instead of compute bounded. 

% To make the learning process feasible, we employ a hierarchical K-means solution. First, the dataset is trained with K-means to get K1 centroids and then the dataset is distributed over obtained Voronoi cells. Second, K2 centroids are trained in each of K1 cells. The final coarse codebook consists of the union of the centroids, a total of $K = K1 \times K2$ centroids.


% % Explanation and analysis
% When $C_1$ is relatively small, the computation time and data transfer time of FC is also small (Equation~\ref{eq2}), whereas the SC execution time is large as for a given number of probes $w$, smaller $C_1$ indicates that there are more vectors to scan (Equation~\ref{eq4}).
% When $C_1$ is large, as the FC execution time is linear in $C_1$ and there are less vectors to scan at SC (for a fixed $w$), the complexity of the entire execution time starts to be dominated by FC. 
% \textbf{Challenge:} Exact search of coarse quantizer centroids can become a bottleneck as $C_1$ increases.
% % Modern architecture has limited memory bandwidth. Given the bandwidth of 59GB/s, it is difficult to reach a few milliseconds latency given these amount of memory accesses.

% \paragraph{Example.}

% Assume....
% The default memory requirement is $1 million \times 128 \times 4$.
% By Equation~\ref{eq5}, the memory requirement is 
% $1 million \times (M \times \frac{Log(C_2)}{8})  + C_1 \times 128 \times 4 + C_2 \times 128 \times 4$. Assume the memory constraint is 1GB, we can use our performance model to get a configuration. We want to maximize recall while staying within 1ms and staying under 1GB of memory requirement. 
% From this analysis, we can come up with the observation that we can use large C1 (\eg, C1 = 65536) as its size is still much smaller than the compressed representation of vectors. 

% We use our memory and performance model for PQ along with our understanding of accuracy trend to answer this question. 
% Choosing C1 : Our performance model shows that when C1 = 14000, the centroid time is 0.114ms. This is already larger than our total latency budget so C1 larger than 14000 can be safely ignored. When C1 = 10,000, our centroid latency is 0.08ms. So we can start our search around with this value.  
% Choosing m and C2 : Now the largest value of m is 100 and largest supported value of C2 = 256. Using these two values,  and C1 = 10,000. The memory requirement is 1.49 GB which is well under our memory requirement. 
% Now we can find a w (number of probes) that gives us the required accuracy. If the centroid scan time is the performance bottleneck, then we can now reduce the centroid to reduce the latency.

% \paragraph{Tradeoffs: Accuracy/Latency/Memory.}

% The higher the number of $C_1$ centroids, the fewer then number of data points we need to scan to achieve a desired level of accuracy. In extreme, when the number of centroid is equal to the number of data points, then   we simply need to scan K-data points to find K-NN. 
% % However, notice that we also need to scan all the centroids.
% For the same number of $C_2$ centroids, the lower the M, the better accuracy and larger memory saving, but also the worse accuracy. This is because...
% $C_2$ is generally very small (\eg, 256) so the $C_2$ codebook size is trivial.
% \minjia{Lead to parameter searching. How to connect the parameter search with the performance model to show its value? }

% \paragraph{Accuracy:}
% The key insight are three folds 

% 	1) The higher the number of C1 centroids, fewer then number of data points we need to scan to achieve a desired level of accuracy. In extreme, when the number of centroid is equal to the number of data points, then   we simply need to scan k-data points to find k-NN. However, notice that we also need to scan all the centroids.
% 	2) For a given number of probes, the accuracy increases as we decrease the number of centroids.
% 3) For the same number  of C2 centroids, higher the m, better the PQ accuracy.  
% Indication:

% \outline{Top-K falls into top-R}

% \paragraph{Observation 3.} For the same number  of C2 centroids, higher the m, better the PQ accuracy.  



% \subsection{Small K vs. Large K of coarse quantizer}
% \outline{Large codebook improves recall but causes first level overhead.}
% \paragraph{Observation 1} The higher the number of C1 centroids, fewer then number of data points we need to scan to achieve a desired level of accuracy. In extreme, when the number of centroid is equal to the number of data points, then   we simply need to scan k-data points to find k-NN. However, notice that we also need to scan all the centroids.
% For a given number of probes, the accuracy increases as we decrease the number of centroids.

% \minjia{Add the on-the-paper analytics here as well.}



